Gradient-Aware Logit Adjustment Loss for Long-tailed Classifier

In the real-world setting, data often follows a long-tailed distribution, where head classes contain significantly more training samples than tail classes. Consequently, models trained on such data tend to be biased toward head classes. The medium of this bias is imbalanced gradients, which include not only the ratio of scale between positive and negative gradients but also imbalanced gradients from different negative classes. Therefore, we propose the Gradient-Aware Logit Adjustment (GALA) loss, which adjusts the logits based on accumulated gradients to balance the optimization process. Additionally, We find that most of the solutions to long-tailed problems are still biased towards head classes in the end, and we propose a simple and post hoc prediction re-balancing strategy to further mitigate the basis toward head class. Extensive experiments are conducted on multiple popular long-tailed recognition benchmark datasets to evaluate the effectiveness of these two designs. Our approach achieves top-1 accuracy of 48.5\%, 41.4\%, and 73.3\% on CIFAR100-LT, Places-LT, and iNaturalist, outperforming the state-of-the-art method GCL by a significant margin of 3.62\%, 0.76\% and 1.2\%, respectively. Code is available at https://github.com/lt-project-repository/lt-project.

==> figures/figure_abla_tau.tex <==
\begin{figure}[t]
\begin{center}
% \vspace{0mm}
\hspace{-3mm}\includegraphics[width=0.48\textwidth]{figures/figure_abla_tau.png}
\end{center}
% \vspace{-4mm}
\caption{Ablation studies on $\tau$. (a) shows the performance over the \textit{many}, \textit{medium} and \textit{few} splits when we use different $\tau$. (b) shows the number of positive predictions over classes(the number of samples classified as its class), when $\tau$ equals different values. The statistics are results from the CIFAR100-LT (}IF=100) testset, where backbone network is ResNet-32.
\label{fig:abla_tau}
% \vspace{-2mm}
\end{figure}

==> figures/teaser_figure_neg_grad.tex <==
\begin{figure*}[t]
\begin{center}
\includegraphics[width=1.0\textwidth]{figures/teaser_figure_neg_grad-1.png}
\end{center}
\vspace{-8mm}
\caption{The overview of the imbalanced negative gradients from different classes. (a) reports the imbalanced negative gradients from different classes of Cross Entropy, EQL, and our GALA loss. (b) illustrates that the smaller negative gradients from tail class samples cannot push the weight of the classifier away enough from these samples. (c) and (d) describe the average similarity between a class weight and features of other head/tail classes when the model is trained with vanilla cross entropy loss and our GALA loss, respectively. The statistics are from experiments performed on CIFAR100-LT (IF=100), where the backbone network is ResNet-32.}
\label{fig:teaser_neg_grad}
\vspace{-1mm}
\end{figure*}

==> figures/teaser_figure_ratio.tex <==
\begin{figure*}[t]
\begin{center}
% \vspace{-2mm}
% \includegraphics[width=1.0\textwidth]{figures/teaser_figure_ratio.png}
\includegraphics[width=1.0\textwidth]{figures/teaser_figure_ratio-1.png}
\end{center}
\vspace{-8mm}
\caption{The overview of the imbalanced ratio of positive and negative gradients. (a) reports the gradient ratio (the ratio of positive to negative gradients) of Cross Entropy, EQL, and our GALA loss. (b) illustrates that due to the imbalanced ratio, the class weight of a classifier is not optimized close to its class. (c) and (d) describe the average similarity between a class weight and features of its class when the model is trained with vanilla cross entropy and our GALA loss, respectively. The statistics are from experiments performed on CIFAR100-LT (IF=100), where the backbone network is ResNet-32.}
\label{fig:teaser_ratio}
\vspace{-1mm}
\end{figure*}

==> sections/2_preliminaries.tex <==
\section{Empirical Analysis}
\label{sec_analysis}
\input{figures/teaser_figure_ratio}
\input{figures/teaser_figure_neg_grad}
In this section, we conduct a series of empirical analyses to examine how the imbalanced positive and negative gradient ratio and negative gradient distribution across classes influence the classification results.
%whethercurrentgraphself-training methodsadoptaprincipledway to leverage unlabeled data for semi-supervised node classification

\noindent \textbf{Empirical Analysis of Imbalanced Gradient Ratio}
We first analyze how the imbalanced positive/negative gradients ratio undermines the optimization of the classifier.
Without loss of generality, we assume the classifier is a feed-forward network where each class has its own learnable weight (i.e., class weight).
Then, we introduce two distinct gradients for a particular class weight: 1) \textit{positive gradients}, obtained from samples of this class, pull this class weight close to samples' features within this class; and 2) \textit{negative gradients}, obtained from samples of other classes, push this class weight away from samples' features of other classes.

We first visualize the relationship between label class (x-axis) and gradient ratio (y-axis) in Fig.~\ref{fig:teaser_ratio}(a). It is clear that the gradient ratio of the tail class is much smaller for EQL and Cross Entropy loss. To further understand how the smaller gradient ratio of the tail class damages the classification results, we visualize the optimization process of the class weight of a tail class A in Fig.~\ref{fig:teaser_ratio}(b). As its illustrated, when the negative gradients overwhelm the positive gradients, the class weight is pushed away from other classes but not necessarily pulled close to sample features of its corresponding class. 
To further verify correlations of a class weight and its features, we visualize their similarity in Fig.\ref{fig:teaser_ratio}(c). 
It shows that the similarity between each tail class weight and the features of its class drops largely, especially in the early training stage.
We can conclude that the imbalanced gradient ratio of tail class weights leads to that samples of tail classes being inclined to be misclassified as other classes. The orange curve in Fig.~\ref{fig:teaser_ratio}(a) and Fig.~\ref{fig:teaser_ratio}(d) show that our GALA loss could balance the gradient ratio and improve the similarity between each tail weight and features of its class.
\iffalse
%%%% Due to the imbalanced data, the gradient for the class vector is imbalanced in two ways:
The imbalanced gradients for class weights impair the classifier in two ways:
(i) 
%%% \textbf{The positive to negative  gradient ratio}(\textbf{the gradient ratio} in short) is imbalanced. 
\textbf{
The imbalanced ratio of positive and negative gradients (called gradient ratio in short) for tail class weights results in
the classifier misclassifying tail class samples as other classes.}
% that the tail class samples cannot be recognized.}
% As shown by the ??color curve of Figure 1(b), since the class contains fewer samples, positive gradient of the weight is much smaller than its the negative gradient.
{As shown by the 
% \textccolor[]{}
\textcolor{blue}{blue curve} in Figure ~\ref{fig:teaser_ratio}(b), since a tail class contains fewer samples, for its class weight the positive gradients are much smaller than negative gradients.}
% As illustrated in Figure 1(a), if the negative gradient overwhelms the positive gradient, the weight are optimized away from other classes but not necessarily updated close to feature of its class. 
{As illustrated in Figure \ref{fig:teaser_ratio}(a), when the negative gradients overwhelm the positive gradients, the class weight is pushed away from other classes but not necessarily pulled close to the samples' features of its class.}
% \weicomment{Pause Marker}
Therefore, the \textcolor{blue}{blue curve} of Figure \ref{fig:teaser_ratio}(c) shows that the similarity between each tail class weight and features of its class drops largely, especially in the early training stage.
We can conclude that the imbalanced gradient ratio of tail class weights leads to that
% its low recognition accuracy on the 
samples of  tail classes are inclined to be misclassified as other classes. 
\fi

\noindent \textbf{Empirical Analysis of Imbalanced Negative Gradient Distribution}
Furthermore, we investigate how the imbalanced negative gradient distribution influences the classification results. 
We first visualize the negative gradient distribution across classes in Fig.\ref{fig:teaser_neg_grad}(a) and discover that the negative gradients from tail class samples are much smaller than the negative gradients from head class samples. 
To further track the root of the problem, Fig.\ref{fig:teaser_neg_grad}(b) illustrates that the smaller negative gradients from other tail class samples cannot push the class weight away enough from these samples.
Taking a further step, we illustrate the similarity of each class weight with head classes and tail class samples in Fig.\ref{fig:teaser_neg_grad}(c) and find that the similarity of each class weight to tail class samples is much higher than that to head class samples.
Thus, the imbalanced negative gradients for a class weight result in that other tail class samples are misclassified as its class. 
In summary, the imbalanced gradients distort the optimization direction of the classifier, making the classifier biased toward head classes.
The orange curve in Fig.~\ref{fig:teaser_neg_grad}(a) and Fig.~\ref{fig:teaser_neg_grad}(d) show that our GALA loss could alleviate the imbalanced negative gradient distribution and the imbalanced similarity to other tail and head classes.


==> tables/tab_iNat.tex <==
\begin{table}[]
% \vspace{-2mm}
\caption{Comparison results on iNaturalist in terms of top-1 accuracy($\%$), where the best and the second best results are shown in \underline{\textbf{underline-bold}} and \textbf{bold}. Except for logit adjustment whose backbone is ResNet-152, the backbone of all other methods is ResNet-50.}
% \vspace{-3mm}
\label{tab_inat}{%

\begin{tabular}{ccccc}
\hline
\multicolumn{1}{c|}{}                               & Many         & Med.         & \multicolumn{1}{c|}{Few}          & Overall        \\ \hline
\multicolumn{1}{c|}{baseline}                       & 72.2         & 63           & \multicolumn{1}{c|}{57.2}         & 61.7           \\
\multicolumn{1}{c|}{LDAM-DRW~\cite{zhang2018mixup}}                 & -            & -            & \multicolumn{1}{c|}{-}            & 68             \\
\multicolumn{1}{c|}{t-Norm~\cite{Kang2020Decoupling}}                   & 65.6         & 65.3         & \multicolumn{1}{c|}{65.5}         & 65.6           \\
\multicolumn{1}{c|}{cRT~\cite{Kang2020Decoupling}}                      & 69           & 66           & \multicolumn{1}{c|}{63.2}         & 65.2           \\
\multicolumn{1}{c|}{BBN~\cite{zhou2020bbn}}                      & 49.4         & 70.8         & \multicolumn{1}{c|}{65.3}         & 66.3           \\
\multicolumn{1}{c|}{TDE~\cite{tang_TDE}}                      & -            & -            & \multicolumn{1}{c|}{-}            & 68.7           \\
\multicolumn{1}{c|}{DisAlign~\cite{Xu2022ConstructingBF}}                 & 69           & 71.1         & \multicolumn{1}{c|}{70.2}         & 70.6           \\
\multicolumn{1}{c|}{MisLAS~\cite{zhong2021improving}}                   & \textbf{73.2}         & \textbf{72.4}         & \multicolumn{1}{c|}{\textbf{70.4}}         & 71.6           \\
\multicolumn{1}{c|}{DRO-LT~\cite{samuel2021distributional}}                   & \textbf{\underline{73.9}}         & 70.6         & \multicolumn{1}{c|}{68.9}         & 69.7           \\
\multicolumn{1}{c|}{DiVE~\cite{He2021DistillingVE}}                     & 70.6         & 70           & \multicolumn{1}{c|}{67.6}         & 69.1           \\
\multicolumn{1}{c|}{Logit adjustment~\cite{menon2021longtail}}         & -            & -            & \multicolumn{1}{c|}{-}            & 71.98          \\
\multicolumn{1}{c|}{Weight Balancing~\cite{alshammari2022long}}                   & 71.2         & 70.4         & \multicolumn{1}{c|}{69.7}         & 70.2           \\
\multicolumn{1}{c|}{DLSA(Bal Soft)~\cite{Xu2022ConstructingBF}}           & -            & -            & \multicolumn{1}{c|}{-}            & 71.6           \\
\multicolumn{1}{c|}{GCL~\cite{li_gcl}}                      & -            & -            & \multicolumn{1}{c|}{-}            & \textbf{72.1}           \\
\multicolumn{1}{c|}{vMF~\cite{Wang2022TowardsCH}}                      & 72.8         & 71.7         & \multicolumn{1}{c|}{70}           & 71             \\ \hline
% \multicolumn{1}{c|}{GALA loss \tiny (ours)}                        & \textbf{73.4}         & 71.4         & \multicolumn{1}{c|}{70.4}         & 71.2             \\
% \multicolumn{1}{c|}{GALA loss + PN \tiny(ours)}                        & 72.6         & \textbf{72.9}         & \multicolumn{1}{c|}{\textbf{73.2}}         & \textbf{73}             \\
\multicolumn{1}{c|}{GALA loss \tiny(ours)}                        & 71.2         & \textbf{\underline{73.2}}         & \multicolumn{1}{c|}{\textbf{\underline{74}}}         & \textbf{\underline{73.3}}             \\ 
\hline
\end{tabular}
}
% \vspace{-1mm}
\end{table}

==> tables/tab_imageNet.tex <==
\begin{table}[]
% \vspace{-0mm}
\caption{Comparison results on ImageNet-LT in terms of top-1 accuracy($\%$), where the best and the second best results are shown in \underline{\textbf{underline-bold}} and \textbf{bold}. The backbone architecture is ResNeXt-50.}
% \vspace{-2mm}
\label{tab_imagenet}
\setlength{\tabcolsep}{1.4mm}{%

\begin{tabular}{ccccc}
\hline
\multicolumn{1}{c|}{}                          & Many           & Med.          & \multicolumn{1}{c|}{Few}           & Overall         \\ \hline
\multicolumn{1}{c|}{baseline}                  & -            & -          & \multicolumn{1}{c|}{-}          & 46.8            \\
\multicolumn{1}{c|}{Focal Loss~\cite{Lin2017FocalLF}}          & \textbf{\underline{67}}             & 41            & \multicolumn{1}{c|}{13.1}          & 47.2            \\
\multicolumn{1}{c|}{LDAM-DRW~\cite{zhang2018mixup}}            & 60             & 49.2          & \multicolumn{1}{c|}{31.9}          & 51.2            \\
\multicolumn{1}{c|}{cRT~\cite{Kang2020Decoupling}}                 & 64.2           & 46.1          & \multicolumn{1}{c|}{26}            & 50.3            \\
\multicolumn{1}{c|}{Balanced Softmax~\cite{ren2020balanced}}               & 62.4           & 47.7          & \multicolumn{1}{c|}{32.1}          & 47.2            \\
\multicolumn{1}{c|}{TDE~\cite{tang_TDE}}                 & 64.9           & 46.9          & \multicolumn{1}{c|}{28.1}          & 51.3            \\
\multicolumn{1}{c|}{MiSLAS~\cite{zhong2021improving}}              & -              & -             & \multicolumn{1}{c|}{-}             & 53.4            \\
\multicolumn{1}{c|}{DRO-LT~\cite{samuel2021distributional}}              & 64             & 49.8          & \multicolumn{1}{c|}{33.1}          & 53.5            \\
\multicolumn{1}{c|}{DiVE~\cite{He2021DistillingVE}}                & 64.06          & 50.41         & \multicolumn{1}{c|}{31.46}         & 53.1            \\
\multicolumn{1}{c|}{Weight Balancing~\cite{alshammari2022long}}              & 62.5           & 50.4          & \multicolumn{1}{c|}{\textbf{ \underline{41.5}}}          & 53.9            \\
\multicolumn{1}{c|}{GCL~\cite{li_gcl}}                 & -              & -             & \multicolumn{1}{c|}{-}             & \textbf{54.88}           \\
\multicolumn{1}{c|}{vMF~\cite{Wang2022TowardsCH}}                 & \textbf{65.9}           & \textbf{50.5}          & \multicolumn{1}{c|}{28.1}          & 53.4            \\ \hline
% \multicolumn{1}{c|}{GALA loss \tiny (ours)}                   & \textbf{66.2}            & 49.6         & \multicolumn{1}{c|} {30.1}         & 53.4           \\
% \multicolumn{1}{c|}{GALA loss + PN \tiny \textbf{ours}} & {65.5}    & \textbf{{51.1}}    & \multicolumn{1}{c|} {{35.8}}          & {54.6}            \\
\multicolumn{1}{c|}{GALA loss \tiny (ours)}     & {63.4}           & \textbf{ \underline{51.8}}    & \multicolumn{1}{c|} {\textbf{39.3}}    & \textbf{\underline{55.0}}         \\ 
\hline 
\end{tabular}
}
% \vspace{-1mm}
\end{table}


==> tables/tab_places.tex <==
\begin{table}[]
% \vspace{-2mm}
\caption{Comparison results on Places-LT in terms of top-1 accuracy($\%$), where the best and the second best results are shown in \underline{\textbf{underline-bold}} and \textbf{bold}. The backbone architecture is ResNet-152.}
% \vspace{-3mm}
\label{tab_places}
{%

\begin{tabular}{c|ccc|c}
\hline
                       & Many & Med. & Few  & Overall \\ \hline
baseline               & \textbf{\underline{45.7}} & 27.3 & 8.2  & 30.2    \\
cRT~\cite{Kang2020Decoupling}              & 42.0 & 37.6 & 24.9 & 36.7    \\
Balanced Softmax~\cite{ren2020balanced} & 41.2 & 39.8 & 31.6 & 38.7    \\
DisAlign~\cite{Xu2022ConstructingBF}         & 40.4 & \textbf{\underline{42.4}} & 30.1 & 39.3    \\
MiSLAS~\cite{zhong2021improving}           & -    & -    & -    & 40.4    \\
DLSA~\cite{Xu2022ConstructingBF}             & 39.7 & 39.2 & \textbf{33.3} & 38.2    \\
GCL~\cite{li_gcl}              & -    & -    & -    & \textbf{40.64}   \\ \hline
% GALA loss \tiny(ours)           & 43.3 & 42.1 & 34.8 & \textbf{41.0}    \\
GALA loss \tiny(ours)      & \textbf{42.4} & \textbf{42.3} & \textbf{\underline{37.8}} & \textbf{\underline{41.4}}   \\ 
\hline
\end{tabular}

}
\end{table}
